Cluster-aware Semi-supervised Learning: Relational Knowledge Distillation Provably Learns Clustering

Despite the empirical success and practical significance of (relational) knowledge distillation that matches (the relations of) features between teacher and student models, the corresponding theoretical interpretations remain limited for various knowledge distillation paradigms. In this work, we take an initial step toward a theoretical understanding of relational knowledge distillation (RKD), with a focus on semi-supervised classification problems. We start by casting RKD as spectral clustering on a population-induced graph unveiled by a teacher model. Via a notion of clustering error that quantifies the discrepancy between the predicted and ground truth clusterings, we illustrate that RKD over the population provably leads to low clustering error. Moreover, we provide a sample complexity bound for RKD with limited unlabeled samples. For semi-supervised learning, we further demonstrate the label efficiency of RKD through a general framework of cluster-aware semi-supervised learning that assumes low clustering errors. Finally, by unifying data augmentation consistency regularization into this cluster-aware framework, we show that despite the common effect of learning accurate clusterings, RKD facilitates a "global" perspective through spectral clustering, whereas consistency regularization focuses on a "local" perspective via expansion.

==> format.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage{hyperref}
\RequirePackage{enumitem}
% \RequirePackage{authblk}

% authblk
% \renewcommand*{\Authsep}{, }
% \renewcommand*{\Authand}{, }
% \renewcommand*{\Authands}{, }
% \renewcommand*{\Affilfont}{\normalsize}
%\renewcommand*{\Authfont}{\bfseries}    % make author names boldface    
% \setlength{\affilsep}{2em}   % set the space between author and affiliation

% enumitem
\setlist{nosep, leftmargin=*}

%%%%%%%%%%%%%%% hyperref %%%%%%%%%%%%%%%
\definecolor{mydarkblue}{rgb}{0,0.08,0.45}
\hypersetup{
    pdftoolbar=true,        % show Acrobat’s toolbar?
    pdfmenubar=true,        % show Acrobat’s menu?
    pdffitwindow=false,     % window fit to page when opened
    pdfstartview={FitH},    % fits the width of the page to the window
    pdftitle={title},    % title
    pdfauthor={Yijun Dong},     % author
    pdfsubject={Subject},   % subject of the document
    pdfcreator={Yijun Dong},   % creator of the document
    pdfproducer={Yijun Dong}, % producer of the document
    % pdfkeywords={}, % list of keywords
    pdfnewwindow=true,      % links in new window
    colorlinks=true,
    linkcolor=mydarkblue,
    citecolor=mydarkblue,
    filecolor=mydarkblue,
    urlcolor=mydarkblue,
}



%%%%%%%%%%%%%%% theorems %%%%%%%%%%%%%%%
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]

\newtheorem{claim}[theorem]{Claim}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}

%\numberwithin{equation}{section}
%\numberwithin{figure}{section}



%%%%%%%%%%%%%%% Special characters %%%%%%%%%%%%%%%
\newcommand{\A}{\mathbb{A}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\C}{\mathbb{C}} % complex field
\newcommand{\D}{\mathbb{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\JJ}{\mathbb{J}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\N}{\mathbb{N}} % nature numbers
\newcommand{\OO}{\mathbb{O}} % nature numbers
\newcommand{\PP}{\mathbb{P}} % nature numbers
\newcommand{\Q}{\mathbb{Q}} % rational field 
\newcommand{\R}{\mathbb{R}} % real field
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\U}{\mathbb{U}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\W}{\mathbb{W}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\Y}{\mathbb{Y}}
\newcommand{\Z}{\mathbb{Z}} % integer field



% bold
\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\renewcommand{\sb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}


\newcommand{\abd}{\boldsymbol{a}}
\newcommand{\bbd}{\boldsymbol{b}}
\newcommand{\cbd}{\boldsymbol{c}}
\newcommand{\dbd}{\boldsymbol{d}}
\newcommand{\ebd}{\boldsymbol{e}}
\newcommand{\fbd}{\boldsymbol{f}}
\newcommand{\gbd}{\boldsymbol{g}}
\newcommand{\hbd}{\boldsymbol{h}}
\newcommand{\ibd}{\boldsymbol{i}}
\newcommand{\jbd}{\boldsymbol{j}}
\newcommand{\kbd}{\boldsymbol{k}}
\newcommand{\lbd}{\boldsymbol{l}}
\newcommand{\mbd}{\boldsymbol{m}}
\newcommand{\nbd}{\boldsymbol{n}}
\newcommand{\obd}{\boldsymbol{o}}
\newcommand{\pbd}{\boldsymbol{p}}
\newcommand{\qbd}{\boldsymbol{q}}
\newcommand{\rbd}{\boldsymbol{r}}
\newcommand{\sbd}{\boldsymbol{s}}
\newcommand{\tbd}{\boldsymbol{t}}
\newcommand{\ubd}{\boldsymbol{u}}
\newcommand{\vbd}{\boldsymbol{v}}
\newcommand{\wbd}{\boldsymbol{w}}
\newcommand{\xbd}{\boldsymbol{x}}
\newcommand{\ybd}{\boldsymbol{y}}
\newcommand{\zbd}{\boldsymbol{z}}

\newcommand{\Abd}{\boldsymbol{A}}
\newcommand{\Bbd}{\boldsymbol{B}}
\newcommand{\Cbd}{\boldsymbol{C}}
\newcommand{\Dbd}{\boldsymbol{D}}
\newcommand{\Ebd}{\boldsymbol{E}}
\newcommand{\Fbd}{\boldsymbol{F}}
\newcommand{\Gbd}{\boldsymbol{G}}
\newcommand{\Hbd}{\boldsymbol{H}}
\newcommand{\Ibd}{\boldsymbol{I}}
\newcommand{\Jbd}{\boldsymbol{J}}
\newcommand{\Kbd}{\boldsymbol{K}}
\newcommand{\Lbd}{\boldsymbol{L}}
\newcommand{\Mbd}{\boldsymbol{M}}
\newcommand{\Nbd}{\boldsymbol{N}}
\newcommand{\Obd}{\boldsymbol{O}}
\newcommand{\Pbd}{\boldsymbol{P}}
\newcommand{\Qbd}{\boldsymbol{Q}}
\newcommand{\Rbd}{\boldsymbol{R}}
\newcommand{\Sbd}{\boldsymbol{S}}
\newcommand{\Tbd}{\boldsymbol{T}}
\newcommand{\Ubd}{\boldsymbol{U}}
\newcommand{\Vbd}{\boldsymbol{V}}
\newcommand{\Wbd}{\boldsymbol{W}}
\newcommand{\Xbd}{\boldsymbol{X}}
\newcommand{\Ybd}{\boldsymbol{Y}}
\newcommand{\Zbd}{\boldsymbol{Z}}


\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}



\newcommand{\Afrak}{\mathfrak{A}}
\newcommand{\Bfrak}{\mathfrak{B}}
\newcommand{\Cfrak}{\mathfrak{C}}
\newcommand{\Dfrak}{\mathfrak{D}}
\newcommand{\Efrak}{\mathfrak{E}}
\newcommand{\Ffrak}{\mathfrak{F}}
\newcommand{\Gfrak}{\mathfrak{G}}
\newcommand{\Hfrak}{\mathfrak{H}}
\newcommand{\Ifrak}{\mathfrak{I}}
\newcommand{\Jfrak}{\mathfrak{J}}
\newcommand{\Kfrak}{\mathfrak{K}}
\newcommand{\Lfrak}{\mathfrak{L}}
\newcommand{\Mfrak}{\mathfrak{M}}
\newcommand{\Nfrak}{\mathfrak{N}}
\newcommand{\Ofrak}{\mathfrak{O}}
\newcommand{\Pfrak}{\mathfrak{P}}
\newcommand{\Qfrak}{\mathfrak{Q}}
\newcommand{\Rfrak}{\mathfrak{R}}
\newcommand{\Sfrak}{\mathfrak{S}}
\newcommand{\Tfrak}{\mathfrak{T}}
\newcommand{\Ufrak}{\mathfrak{U}}
\newcommand{\Vfrak}{\mathfrak{V}}
\newcommand{\Wfrak}{\mathfrak{W}}
\newcommand{\Xfrak}{\mathfrak{X}}
\newcommand{\Yfrak}{\mathfrak{Y}}
\newcommand{\Zfrak}{\mathfrak{Z}}


% Greek
\newcommand{\eps}{\epsilon}
\newcommand{\veps}{\varepsilon}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\deltab}{\boldsymbol{\delta}}
\newcommand{\epsb}{\boldsymbol{\eps}}
\newcommand{\vepsb}{\boldsymbol{\veps}}
\newcommand{\zetab}{\boldsymbol{\zeta}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\vthetab}{\boldsymbol{\vartheta}}
\newcommand{\iotab}{\boldsymbol{\iota}}
\newcommand{\kappab}{\boldsymbol{\kappa}}
\newcommand{\vkappab}{\boldsymbol{\varkappa}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\nub}{\boldsymbol{\nu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\omicronb}{\boldsymbol{\omicron}}
\newcommand{\pib}{\boldsymbol{\pi}}
\newcommand{\vpib}{\boldsymbol{\varpi}}
\newcommand{\rhob}{\boldsymbol{\rho}}
\newcommand{\vrhob}{\boldsymbol{\varrho}}
\newcommand{\sigmab}{\boldsymbol{\sigma}}
\newcommand{\vsigmab}{\boldsymbol{\varsigma}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\upsilonb}{\boldsymbol{\upsilon}}
\newcommand{\phib}{\boldsymbol{\phi}}
\newcommand{\vphib}{\boldsymbol{\varphi}}
\newcommand{\chib}{\boldsymbol{\chi}}
\newcommand{\psib}{\boldsymbol{\psi}}
\newcommand{\omegab}{\boldsymbol{\omega}}

\newcommand{\Alphab}{\boldsymbol{\Alpha}}
\newcommand{\Betab}{\boldsymbol{\Beta}}
\newcommand{\Gammab}{\boldsymbol{\Gamma}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Epsb}{\boldsymbol{\Epsilon}}
\newcommand{\Zetab}{\boldsymbol{\Zeta}}
\newcommand{\Etab}{\boldsymbol{\Eta}}
\newcommand{\Thetab}{\boldsymbol{\Theta}}
\newcommand{\Iotab}{\boldsymbol{\Iota}}
\newcommand{\Kappab}{\boldsymbol{\Kappa}}
\newcommand{\Lambdab}{\boldsymbol{\Lambda}}
\newcommand{\Mub}{\boldsymbol{\Mu}}
\newcommand{\Nub}{\boldsymbol{\Nu}}
\newcommand{\Xib}{\boldsymbol{\Xi}}
\newcommand{\Omicronb}{\boldsymbol{\Omicron}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\Rhob}{\boldsymbol{\Rho}}
\newcommand{\Sigmab}{\boldsymbol{\Sigma}}
\newcommand{\Taub}{\boldsymbol{\Tau}}
\newcommand{\Upsilonb}{\boldsymbol{\Upsilon}}
\newcommand{\Phib}{\boldsymbol{\Phi}}
\newcommand{\Chib}{\boldsymbol{\Chi}}
\newcommand{\Psib}{\boldsymbol{\Psi}}
\newcommand{\Omegab}{\boldsymbol{\Omega}}








%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand{\dfeq}{\triangleq}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
\newcommand{\pinv}{\dagger}
\newcommand*{\poly}{\mathop{\mathrm{poly}}}
\newcommand*{\mean}{\mathop{\mathrm{mean}}}
\newcommand*{\median}{\mathop{\mathrm{median}}}
\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\range}{\mathop{\mathrm{Range}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\prox}{\mathop{\mathrm{prox}}}
\newcommand{\proj}{\mathop{\mathrm{proj}}}
\newcommand{\spn}{\mathop{\mathrm{span}}}
\newcommand{\row}{\mathop{\mathrm{row}}}
\newcommand{\col}{\mathop{\mathrm{col}}}
\renewcommand{\mod}{\mathop{\mathrm{mod}}}
\newcommand{\nucnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
\newcommand{\pto}{\mathrel{\ooalign{\hfil$\mapstochar\mkern5mu$\hfil\cr$\to$\cr}}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}

\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{\partial #1^2}}
\newcommand{\pnwrt}[2]{\frac{\partial^#1}{\partial #2^#1}}
\newcommand{\pfrac}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ppfrac}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\pnfrac}[3]{\frac{\partial^#1 #2}{\partial #3^#1}}

% \newcommand{\eproof}{$\null\hfill\blacksquare$}
% \renewcommand\qedsymbol{$\blacksquare$}



%%%%%%%%%%%%%%% Super/sup-scripts %%%%%%%%%%%%%%%
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\ol}[1]{\overline{#1}} % overline
\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}




%%%%%%%%%%%%%%% Short Forms %%%%%%%%%%%%%%%
\newcommand{\ea}{\emph{et al.}\xspace}
\newcommand{\eg}{\emph{e.g.}\xspace}
\newcommand{\ie}{\emph{i.e.}\xspace}
\newcommand{\iid}{\emph{i.i.d.}\xspace}
\newcommand{\cf}{\emph{cf.}\xspace}
\newcommand{\wrt}{\emph{w.r.t.}\xspace}
\newcommand{\st}{\emph{s.t.}\xspace}
\newcommand{\whp}{\emph{w.h.p.}\xspace}



%%%%%%%%%%%%%%% Brackets %%%%%%%%%%%%%%
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abbr}[1]{\left\vert#1\right\vert}
\newcommand{\abr}[1]{\langle#1\rangle}
\newcommand{\nnbr}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\newcommand{\rsep}[2]{\left(#1 \middle\vert #2 \right)}
\newcommand{\ssep}[2]{\left[#1 \middle\vert #2 \right]}
\newcommand{\csep}[2]{\left\{#1 \middle\vert #2 \right\}}
\newcommand{\asep}[2]{\langle#1 \middle\vert #2 \rangle}
\newcommand{\rsepp}[2]{\left(#1 ~\middle\vert~ #2 \right)}
\newcommand{\ssepp}[2]{\left[#1 ~\middle\vert~ #2 \right]}
\newcommand{\csepp}[2]{\left\{#1 ~\middle\vert~ #2 \right\}}
\newcommand{\asepp}[2]{\langle#1 ~\middle\vert~ #2 \rangle}

\newcommand{\apar}[1]{\langle #1 \rangle}
\newcommand{\cpar}[1]{\{#1\}}
\newcommand{\bpar}[1]{\Big( #1 \Big)}
\newcommand{\Bpar}[1]{\Bigg( #1 \Bigg)}
\newcommand{\bspar}[1]{\Big[ #1 \Big]}
\newcommand{\Bspar}[1]{\Bigg[ #1 \Bigg]}
\newcommand{\bcpar}[1]{\Big\{ #1 \Big\}}
\newcommand{\Bcpar}[1]{\Bigg\{ #1 \Bigg\}}

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\inpr}[2]{\langle #1, #2 \rangle}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\mat}[1]{\begin{pmatrix} #1 \end{pmatrix}}


%%%%%%%%%%%%%%% Python %%%%%%%%%%%%%%%
\definecolor{commentcolor}{RGB}{110,154,155}   % define comment color
\newcommand{\PyComment}[1]{\ttfamily\textcolor{commentcolor}{\# #1}}  % add a "#" before the input text "#1"
\newcommand{\PyCode}[1]{\ttfamily\textcolor{black}{#1}} % \ttfamily is the code font


%%%%%%%%%%%%%%% Miscellaneous %%%%%%%%%%%%%%%
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\bs}[1]{\boldsymbol{#1}}
\renewcommand{\b}{\textbf}
\renewcommand{\t}[1]{\text{#1}}
% starred section table of contents
\newcommand{\sectiontoc}[1]{
\section*{#1}
\addcontentsline{toc}{section}{\protect\numberline{}#1}%
}




% Local
\newcommand{\QL}[1]{\red{[Qi: #1]}}
\newcommand{\yd}[1]{\blue{[yijun: #1]}}
\newcommand{\km}[1]{\textcolor{cyan}{[kevin: #1]}}
\newcommand{\needref}{\textcolor{red}{\textbf{@@ref}}}
\newcommand{\iffun}[1]{\mathbbm{1}\cbr{#1}}
\newcommand{\unif}{\mathop{\mathrm{Unif}}}
\newcommand{\onehot}[1]{\overrightarrow{#1}}
\newcommand{\rademacher}{\mathop{\mathrm{Rad}}}
\newcommand{\nbhd}{\mathop{\mathrm{NB}}}
\newcommand{\softmax}{\mathop{\mathtt{softmax}}}

\newcommand{\Flap}[1]{\Fcal_{\Lb\rbr{#1}}}
\newcommand{\Fdac}[1]{\Fcal^{\tau}_{#1}}

\newcommand{\repfun}{\psi}
\newcommand{\repker}{k_{\repfun}}

\newcommand{\lossemp}{\wh\Ecal}
\newcommand{\losspop}{\Ecal}

\newcommand{\reglappop}{R} 
\newcommand{\reglapemp}[1]{\wh{\reglappop}_{#1}}
\newcommand{\reglapempse}[1]{\wh{\reglappop}^{\mathrm{se}}_{#1}}
\newcommand{\reglapu}[1]{\wh{r}_{#1}}
\newcommand{\regdac}[1]{\wh{\Lcal}^\dac_{#1}}
\newcommand{\lossce}[1]{\wh{\Lcal}^\ce_{#1}}

\newcommand{\flapemp}{f_{\vert \Xb^u}}
\newcommand{\flappop}{f_{\vert \Xcal}}
\newcommand{\flapempse}{f^{\mathrm{se}}_{\vert \Xb^u}}
\newcommand{\hflapemp}{\wh{f}_{\vert \Xb^u}}
\newcommand{\hflappop}{\wh{f}_{\vert \Xcal}}

% constants
\newcommand{\fgtice}{\alpha} % fraction of ground truth inter-class edge weights
\newcommand{\bdf}{B_f}
\newcommand{\bdker}{B_{\repker}}

\newcommand{\ce}{\mathrm{CE}}
\newcommand{\rkd}{\mathrm{RKD}}
\newcommand{\dac}{\mathrm{DAC}}
